Agent That Debugs: Dynamic State-Guided Vulnerability Repair

In recent years, more vulnerabilities have been discovered every day, while manual vulnerability repair requires specialized knowledge and is time-consuming. As a result, many detected or even published vulnerabilities remain unpatched, thereby increasing the exposure of software systems to attacks. Recent advancements in agents based on Large Language Models have demonstrated their increasing capabilities in code understanding and generation, which can be promising to achieve automated vulnerability repair. However, the effectiveness of agents based on static information retrieval is still not sufficient for patch generation. To address the challenge, we propose a program repair agent called VulDebugger that fully utilizes both static and dynamic context, and it debugs programs in a manner akin to humans. The agent inspects the actual state of the program via the debugger and infers expected states via constraints that need to be satisfied. By continuously comparing the actual state with the expected state, it deeply understands the root causes of the vulnerabilities and ultimately accomplishes repairs. We experimentally evaluated VulDebugger on 50 real-life projects. With 60.00% successfully fixed, VulDebugger significantly outperforms state-of-the-art approaches for vulnerability repair.

==> components/background.tex <==
\section{Crash-free Constraint}
\label{sec:background}

%Before presenting the technical details, let us first provide some
%background on crash-free constraints.

% \subsection{LLM-related Technologies}
% \xiang{I feel this subsection should be moved to related work}
% Large language models (LLMs) have facilitated new breakthroughs in various research fields. Additionally, their capabilities in code understanding and generation have shown promising results in software engineering tasks. However, the effectiveness of zero-shot approaches in problem-solving with large models has been unsatisfactory. To enhance the capabilities of LLMs in code-related tasks, existing research has already introduced various proven techniques. 
% %Researchers have now made significant progress on LLMs, but there are still many shortcomings in the implementation of specific tasks.
% %To solve the problem, 

% \textbf{Chain-of-thought.} 
% Chain-of-thought prompting\citep{wei2022chain} (CoT) has been proposed to improve the ability of large language models to perform complex reasoning. CoT enables LLMs to elicit multi-step reasoning behavior by decomposing multi-step problems into intermediate steps, which improves performance by a large margin on arithmetic reasoning.
% Secondly, the CoT provides an interpretable window into the model's behavior, illustrating how it arrives at specific answers and offering opportunities to identify and debug errors in the reasoning path.

% \textbf{LLM-based agent.} LLM-based agents represent an innovative application of its capabilities, autonomously planning and executing actions to fulfill specific objectives. The fundamental mechanism involves providing the LLM with a prompt detailing the current state of the environment, the desired goal, and possible subsequent actions. The model then determines the most appropriate action to take. Feedback from the executed action is assimilated back into the model for refining future prompts, thereby enhancing the decision-making process in subsequent iterations.

% \textbf{Retrieval-augmented generation.} 
% Retrieval-Augmented Generation (RAG) is a model architecture that combines information retrieval with text generation, which improves the quality and accuracy of text generation~\citep{jiang2024survey}. 
% %Then researchers try to drive LLMs to access program static information by using API calls. 
% Currently, the RAG technology has been implemented in numerous tasks driven by LLMs. 
% In the field of LLM for software engineering, RAG technology is commonly used to retrieve information from the internet to augment the knowledge of LLMs, or to access code repository information to enhance LLMs' overall understanding of code~\citep{zhang2024llm, liu2024codexgraph, zhang2023repocoder, pan2024enhancing, arora2024masai}.
% For example, Zhang et al.\citep{zhang2024autocoderover} propose \autocoderover where the program is represented as an abstract syntax tree to enhance LLM's understanding of the issue's root cause. The approach of using RAG technology to retrieve static code information provides static insights for software engineering tasks. However, this method alone is insufficient for effectively completing vulnerability repair tasks. To enable LLMs to accurately perform vulnerability repairs, additional critical information is necessary.


%\subsection{Crash-free Constraint}
\citet{gao2021beyond} propose \ExtractFix{} based on extracting crash-free constraint (CFC). 
To prevent recurrent crashes at the same location, a CFC can be deduced and enforced. 
The CFC encapsulates conditions that, when satisfied, ensure that the location in question does not lead to a crash. 
For example, the CFC for a null-pointer dereference of \(p\) might be that the pointer is non-null (\(p \neq 0\)), and for array access errors in \(a[i]\), it ensures that the index is within bounds (\(i < \text{SIZE}\)). 
By modifying the program to consistently satisfy the CFC at critical points, it is ensured that the same crash will not occur under any input, thereby making the CFC a safeguard against the violation of crucial program properties for all inputs. 
This property of the CFC aligns remarkably with the characteristics of the expected states in the debugging process. Consequently, we consider the CFC to be an excellent concept for indicating the expected states of a program.
%Extracted with the aid of sanitizer, CFC is the symbolization or abstraction of the concrete violations, where stores the expected state of the program at the point. LLMs can compare the real state with the expected state to better find out the root cause and localize, thus correctly generating patch.  
